SPARC: Scenario Planning and Reasoning for Automated C Unit Test Generation

Automated unit test generation for C remains a formidable challenge due to the semantic gap between high-level program intent and the rigid syntactic constraints of pointer arithmetic and manual memory management. While Large Language Models (LLMs) exhibit strong generative capabilities, direct intent-to-code synthesis frequently suffers from the leap-to-code failure mode, where models prematurely emit code without grounding in program structure, constraints, and semantics. This will result in non-compilable tests, hallucinated function signatures, low branch coverage, and semantically irrelevant assertions that cannot properly capture bugs. We introduce SPARC, a neuro-symbolic, scenario-based framework that bridges this gap through four stages: (1) Control Flow Graph (CFG) analysis, (2) an Operation Map that grounds LLM reasoning in validated utility helpers, (3) Path-targeted test synthesis, and (4) an iterative, self-correction validation loop using compiler and runtime feedback. We evaluate SPARC on 59 real-world and algorithmic subjects, where it outperforms the vanilla prompt generation baseline by 31.36% in line coverage, 26.01% in branch coverage, and 20.78% in mutation score, matching or exceeding the symbolic execution tool KLEE on complex subjects. SPARC retains 94.3% of tests through iterative repair and produces code with significantly higher developer-rated readability and maintainability. By aligning LLM reasoning with program structure, SPARC provides a scalable path for industrial-grade testing of legacy C codebases.

==> sections/discussion.tex <==
\section{Discussion}

==> tables/combined_5_6.tex <==
\begin{figure*}[t]
  % \begin{minipage}[t]{0.74\textwidth}
    \vspace{0pt}
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l|c|ccc|ccc|ccc|ccc|ccc}
    \toprule
    \multirow{2}{*}{\textbf{Identifier}} & \multirow{2}{*}{\textbf{\#Paths}} & \multirow{2}{*}{\textbf{\#Function}} & \multirow{2}{*}{\textbf{\#Line}} & \multirow{2}{*}{\textbf{\#Branch}} & \multicolumn{3}{c|}{\textbf{Function Cov. (\%)}} & \multicolumn{3}{c|}{\textbf{Line Cov. (\%)}} & \multicolumn{3}{c|}{\textbf{Branch Cov. (\%)}} & \multicolumn{3}{c}{\textbf{Mutation Score (\%)}} \\
    \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} \cmidrule(lr){15-17}
    & & & & & DeepSeek & Gemini & GPT-5 & DeepSeek & Gemini & GPT-5 & DeepSeek & Gemini & GPT-5 & DeepSeek & Gemini & GPT-5 \\
    \midrule
    alaw & 17 & 11 & 74 & 34 & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & 95.90 & \textbf{100.00} & \textbf{100.00} & 82.40 & \textbf{100.00} & 97.06 & 62 & \textbf{77} & 65 \\
    affine & 25 & 12 & 95 & 40 & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & 86.30 & 96.84 & \textbf{100.00} & 85.00 & \textbf{95.00} & \textbf{95.00} & 44 & 59 & \textbf{74} \\
    decimal\_to\_any\_base & 21 & 9 & 61 & 40 & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & \textbf{95.10} & 95.08 & 95.08 & \textbf{72.50} & 70.00 & 70.00 & 72 & \textbf{75} & \textbf{75} \\
    infix\_to\_postfix & 35 & 14 & 117 & 110 & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & 79.50 & 79.49 & \textbf{80.34} & 69.10 & \textbf{70.00} & \textbf{70.00} & \textbf{76} & 65 & 70 \\
    lcs & 20 & 11 & 100 & 76 & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & 93.00 & \textbf{95.00} & 91.00 & \textbf{85.50} & 75.00 & 71.05 & \textbf{69} & 58 & 57 \\
    ascending\_priority\_queue & 36 & 15 & 143 & 92 & \textbf{100.00} & 86.67 & \textbf{100.00} & 91.60 & 72.03 & \textbf{93.01} & 79.30 & 61.96 & \textbf{79.35} & 69 & \textbf{74} & \textbf{74} \\
    binary\_search\_tree & 26 & 8 & 76 & 44 & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & \textbf{98.70} & 98.68 & 98.68 & \textbf{93.20} & 93.18 & 90.91 & \textbf{74} & \textbf{74} & 69 \\
    doubly\_linked\_list & 12 & 5 & 79 & 44 & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & \textbf{97.40} & 77.22 & 58.23 & \textbf{86.40} & 65.91 & 43.18 & \textbf{81} & 56 & 37 \\
    dynamic\_stack & 61 & 16 & 161 & 128 & \textbf{93.80} & 87.50 & 87.50 & 85.10 & \textbf{87.58} & 86.96 & 68.80 & \textbf{70.31} & 69.53 & \textbf{70} & \textbf{70} & 69 \\
    prime\_factorization & 29 & 9 & 126 & 76 & \textbf{100.00} & \textbf{100.00} & \textbf{100.00} & \textbf{76.20} & 70.63 & 73.81 & 75.00 & \textbf{76.32} & 75.00 & 52 & 55 & \textbf{57} \\
    \midrule
    \textbf{Total/Average} & 284 & 110 & 1,032 & 684 & \textbf{99.38} & 97.42 & 98.75 & \textbf{89.88} & 87.26 & 87.71 & \textbf{79.72} & 77.77 & 76.11 & \textbf{66.90} & 66.30 & 64.70 \\
    \bottomrule
    \end{tabular}%
    }
    \captionof{table}{Coverage comparison across \texttt{DeepSeek~V3.2}, \texttt{Gemini 3 Flash Preview}, and \texttt{GPT-5-Mini}}
    \label{tab:llm_selection}
  % \end{minipage}%
  % \hfill
  % \begin{minipage}[t]{0.25\textwidth}
  %   \vspace{0pt}
  %   \centering
  %   \includegraphics[width=\textwidth]{figures/rq51_scalability.png}
  %   \captionof{figure}{Token usage vs. identifier complexity.}
  %   \label{fig:rq51_scalability}
  % \end{minipage}
\end{figure*}


